Two-particle azimuthal correlations at forward rapidity in STAR

During the 2008 run the Relativistic Heavy Ion Collider (RHIC) at the Brookhaven Nation Laboratiory (BNL), NY, provided high luminosity in both p+p and d+Au collisions at $\sqrt{s_{NN}}=200\mathrm{\,GeV}$. Electromagnetic calorimeter acceptance in STAR was enhanced by the new Forward Meson Spectrometer (FMS), and is now almost contiguous from $-1<\eta\4$ over the full azimuth. This allows measurements of the azimuthal correlation between a forward neutral pion and a second particle in a very large rapidity range. Di-hadron azimuthal correlations provide sensitivity to the low longitudinal momentum fraction ($x$) component of the gluon density in the nuclear target. Initial state nonlinear effects are in fact expected to appear in d+Au collisions when the dense part of the nucleus is probed. The analysis in this thesis shows that such correlations and their dependence on rapidity, transverse momentum and collision centrality are qualitative consistent with the existence of gluon saturation effects in the relativistic nucleus. Theoretical expectations for azimuthal correlations between a dilute system (deuteron) and a saturated target (Gold nucleus) have been explored.

==> TitlePage.tex <==
\begin{titlepage}
\begin{center}
\noindent {\large \textbf{UNIVERSITY OF NICE - SOPHIA ANTIPOLIS}} \\
\vspace*{0.3cm}
\noindent {\LARGE \textbf{DOCTORAL SCHOOL STIC}} \\
\noindent \textbf{SCIENCES ET TECHNOLOGIES DE L'INFORMATION \\ ET DE LA COMMUNICATION} \\
\vspace*{0.5cm}
\noindent \Huge \textbf{P H D\ \ T H E S I S} \\
\vspace*{0.3cm}
\noindent \large {to obtain the title of} \\
\vspace*{0.3cm}
\noindent \LARGE \textbf{PhD of Science} \\
\vspace*{0.3cm}
\noindent \Large of the University of Nice - Sophia Antipolis \\
\noindent \Large \textbf{Specialty : \textsc{Computer Science}}\\
\vspace*{0.4cm}
\noindent \large {Defended by\\}
\noindent \LARGE Olivier \textsc{Commowick} \\
\vspace*{0.8cm}
\noindent {\Huge \textbf{Design and Use of Aatomical Atlases for Radiotherapy}} \\
\vspace*{0.8cm}
\noindent \Large Thesis Advisor: Grégoire \textsc{Malandain} \\
\vspace*{0.2cm}
\noindent \Large prepared at INRIA Sophia Antipolis, \textsc{Asclepios} Team\\
\vspace*{0.2cm}
\noindent \large defended on February 14, 2007 \\
\vspace*{0.5cm}
\end{center}
\noindent \large \textbf{Jury :} \\
\begin{center}
\noindent \large 
\begin{tabular}{llcl}
      \textit{Reviewers :}	& Patrick \textsc{Clarysse}		& - & CNRS (CREATIS)\\
				& Louis \textsc{Collins}		& - & McGill University\\
      \textit{Advisor :}	& Grégoire \textsc{Malandain}		& - & INRIA (Asclepios)\\
      \textit{President :}	& Nicholas \textsc{Ayache}		& - & INRIA (Asclepios)\\
      \textit{Examinators :}   & Pierre-Yves \textsc{Bondiau}          & - & Centre Antoine Lacassagne (Nice)\\
      				& Guido \textsc{Gerig}			& - & University of North Carolina\\
      				& Vincent \textsc{Grégoire}		& - & Université Catholique de Louvain\\
      \textit{Invited :}		& Hanna \textsc{Kafrouni}		& - & DOSISoft S.A.
\end{tabular}
\end{center}
\end{titlepage}
\sloppy

\titlepage


==> chapter_5.tex <==

%%% Chapter heading commands %%%

\chapter{Systematics and yield extraction}\label{chapter_systematics}

Mid-rapidity particles used to compute the azimuthal correlation with a forward $\pi^{0}$ have been selected using the same kinematical cuts and within the same acceptance. The reason for this is to compare $\pi^{0}-\pi^{0}$ (FMS-BEMC) and $\pi^{0}-h^{\pm}$ (FMS-TPC) correlations in order to look for consistencies in the broadening effect. In order to being able to compare such quantities, some corrections regarding efficiency and background subtraction need to be applied to both correlations. In this chapter we will discuss the necessary corrections to apply to the reconstruction of TPC tracks and BEMC neutral pions. Since all correlations are normalized per trigger pions, inefficiencies related to the FMS pion reconstruction will cancel out in this comparison; therefore, FMS corrections will not be discussed at this point. Similarly, vertex inefficiencies cancel out as well, since the same vertex requirement is applied to both correlation measurements.

\section{FMS-TPC correlations}

Reconstruction of charged tracks in the TPC proves to be relatively clean. The tracking efficiency depends on the acceptance of the detector and the detection efficiency. The TPC acceptance is $\mathrm{96\%}$ for tracks traveling perpendicular to the beamline \cite{Anderson2003659}. The $\mathrm{4\%}$ inefficiency is caused by spaces between the TPC sectors. The total reconstruction efficiency, including the TPC acceptance, is estimated from the number of associated tracks in the reconstructed Monte-Carlo events. The efficiency has been studied for different species of charged hadrons \cite{Ruan:2005hy} and it proves to be fairly constant in $p_{T}$ for particles with $p_{T}>0.3\mathrm{\,GeV/c}$ (Figure \ref{5.tpceff}), as well as not dependent on the pseudo-rapidity. The TPC efficiency is therefore taken to be a constant value of $\epsilon_{TPC}=90\%$ for both p+p and d+Au interactions. 

\begin{figure}\label{5.tpceff}
\begin{tabular}{c c}
\includegraphics[width=0.5\textwidth]{figures/chapter5/pluseff.eps} 
\includegraphics[width=0.5\textwidth]{figures/chapter5/minuseff.eps} 
\end{tabular}
\caption{TPC reconstruction efficiency of $\pi^{\pm}$, $K^{\pm}$, $p$ and $\bar{p}$ as a function of $p_{T}$. Positive (negative) charged particles are on the left (right). Figure from \cite{Ruan:2005hy}.}
\end{figure}

Although the TPC allows a relatively clean and efficient reconstruction of charged tracks, its slow readout time, much slower than the bunch crossing time, may cause many of the tracks to be actually from piled up collisions. When this happens, multiple vertexes are found in the event. In cases where the piled up vertex is generated from earlier or later bunch crossings, the tracks topology shows discontinuity at the TPC central membrane. Such cases are recognized by the vertex finding algorithm \cite{Reed:2010zz} and the vertex is rejected. When the piled up collision happen within the same bunch crossing, the vertexes have the same quality and it is more difficult to disentangle them. For this reason, it is necessary to apply a correction for piled up events to the azimuthal correlations. Since the average number of pile up events is proportional to the instantaneous luminosity, in order to estimate such contribution, it is useful to study the variation of the $\Delta\varphi$ distribution with the luminosity. Production runs have been divided in three luminosity classes, based on BBC rates, labeled as low ($\langle\mathcal{R}^{BBC}_{pp}\rangle=269\mathrm{\,KHz}$ and $\langle\mathcal{R}_{dAu}^{BBC}\rangle=128\mathrm{\,KHz}$), mid ($\langle\mathcal{R}^{BBC}_{pp}\rangle=334\mathrm{\,KHz}$ and $\langle\mathcal{R}^{BBC}_{dAu}\rangle=173\mathrm{\,KHz}$) and high luminosity ($\langle\mathcal{R}^{BBC}_{pp}\rangle=416\mathrm{\,KHz}$ and $\langle\mathcal{R}^{BBC}_{dAu}\rangle=234\mathrm{\,KHz}$). Azimuthal correlation have been measured for these three run selections and results (for one set of $p_{T}$ cuts) are show in Figure \ref{5.lumi}. Table \ref{5.lumitable} shows instead the values of the correlated signal yield $A$ and standard deviation $\sigma$ and the uncorrelated constant background $b$, as obtained from the fit on data. While signal yields and widths does not change, as expected, with luminosity, the uncorrelated background increases with increasing luminosity. Such effect is larger in p+p, where the luminosity is larger, than in d+Au interactions. To correct for this uncorrelated pile up contribution, it is useful to extrapolate the background level at zero luminosity (right-hand plot in Figure \ref{5.lumi}). The contribution that exceed this value corresponds to pile up to the coincidence probability and has to be subtracted from the azimuthal correlations. Once this constant (uncorrelated) background is subtracted from the coincidence probability, the distribution can be corrected for the TPC efficiency. 

\begin{figure}\label{5.lumi}
\begin{tabular}{c c}
\includegraphics[width=0.45\textwidth]{figures/chapter5/luminosity1.eps} 
\includegraphics[width=0.45\textwidth]{figures/chapter5/luminosity2.eps} 
\end{tabular}
\caption{Uncorrected inclusive azimuthal correlations for three luminosity classes (lower to the left, higher to the right) for higher $p_{T}$ selection of p+p (top) and d+Au (bottom row) collisions. The right panels show the uncorrelated background component, as extrapolated from the fit, versus the luminosity.}
\end{figure}

\begin{table}\label{5.lumitable}\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline int. & $ p_{T} $ cuts & $\langle\mathcal{R}^{BBC}\rangle$ & A & $\sigma$ & b & b(0) \\ \hline\hline 
\multirow{6}{*}{p+p} & \multirow{3}{*}{higher} & low & $0.097\pm0.008$ & $0.736\pm0.061$ & $0.019\pm0.001$ & \multirow{3}{*}{$0.011\pm0.005$}  \\ 
& & mid & $0.098\pm0.007$ & $0.829\pm0.055$ & $0.021\pm0.001$ & \\ 
& & high & $0.089\pm0.010$ & $0.710\pm0.082$ & $0.023\pm0.002$ & \\ \cline{2-7}
& \multirow{3}{*}{lower} & low & $0.211\pm0.012$ & $0.856\pm0.043$ & $0.081\pm0.002$ &\multirow{3}{*}{$0.060\pm0.008$}\\
& & mid & $0.213\pm0.010$ & $0.827\pm0.034$ & $0.087\pm0.002$&   \\ 
& & high & $0.230\pm0.017$ & $0.866\pm0.061$ & $0.092\pm0.003$& \\ \hline
\multirow{6}{*}{d+Au} & \multirow{3}{*}{higher} & low & $0.104\pm0.009$ & $0.798\pm0.056$ & $0.098\pm0.002$ & \multirow{3}{*}{$0.080\pm0.005$}  \\ 
& & mid & $0.107\pm0.009$ & $0.811\pm0.058$ & $0.100\pm0.002$ & \\ 
& & high & $0.096\pm0.010$ & $0.759\pm0.073$ & $0.110\pm0.002$ &\\ \cline{2-7}
& \multirow{3}{*}{lower} & low & $0.251\pm0.013$ & $0.850\pm0.036$ & $0.334\pm0.002$ & \multirow{3}{*}{$0.276\pm0.006$} \\
& & mid & $0.262\pm0.014$ & $0.960\pm0.042$ & $0.347\pm0.003$ & \\ 
& & high & $0.243\pm0.018$ & $0.947\pm0.056$ & $0.377\pm0.003$ &\\ \hline 
\end{tabular}\caption{Summary.}\end{center}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{FMS-BEMC correlations}

The reconstruction of mid-rapidity neutral pions is characterized by larger uncertainties than charged tracks. The main source of such uncertainties is the presence of a significant background in the invariant mass spectrum of the pion candidates. The subtraction of a background component from the correlation distributions (background pair - forward pion correlation) is therefore necessary before applying any efficiency correction. In order to estimate the background contribution and to calculate the reconstruction efficiency and the detector acceptance, a simulation of one million minimum bias p+p events have been produced by PYTHIA, using GSTAR to simulate the detector responses., as well as a one million d+Au events using HIJING+GEANT. The choice of a minimum bias, instead of a simulation of events presenting a forward trigger $\pi^{0}$ within the FMS acceptance, has been made, for practical reasons, in order to enhance the statistics at mid-rapidity. The $z$ component of the vertex has been randomly smeared (using a Gaussian noise with $\sigma=30\mathrm{\,cm}$) in simulation, in order to emulate the BBC vertex reconstruction uncertainty. The calibration table used for the simulation has been chosen in order to best represent the average BEMC configuration during the run. 

\begin{figure}\label{5.multiplicitycomparison}
\begin{tabular}{c c}
\includegraphics[width=0.45\textwidth, height=0.45\textwidth, clip=]{figures/chapter5/plt.eps} 
\includegraphics[width=0.45\textwidth, height=0.45\textwidth]{figures/chapter5/clustermulti.eps} 
\end{tabular}
\caption{Left: number of charged hadrons plus photons from $\pi^{0}$ decay, as simulated in minimum bias (top) and forward triggered PYTHIA events (bottom). Right: cluster multiplicity comparison between minimum bias PYTHIA+GEANT simulation (top) and forward triggered data (bottom).}
\end{figure}

\begin{figure}\label{5.comparisonsimu}
\begin{tabular}{c c}
\includegraphics[width=0.45\textwidth]{figures/chapter5/comparison.eps} 
\includegraphics[width=0.45\textwidth]{figures/chapter5/comparison2.eps} 
\end{tabular}
\caption{Simulation-Data comparison for $\pi^{0}$ parameters ($p_{T}$, $Z_{\gamma\gamma}$, $\eta$, $\varphi$) in p+p (left) and d+Au interactions (right). }
\end{figure}

\begin{figure}\label{5.masse}
\begin{tabular}{c c}
\includegraphics[width=0.45\textwidth]{figures/chapter5/masseffect.eps} 
\includegraphics[width=0.45\textwidth]{figures/chapter5/masseffect2.eps} 
\end{tabular}
\caption{Simulation-Data comparison between invariant mass distributions for BEMC cluster pairs  for different $p_{T}$ selections, in p+p (left) and d+Au interactions (right).}
\end{figure}

The main difference between simulation and data is represented by the higher multiplicity in forward triggered events compared to the minimum bias simulation. This is indeed expected from pure PYTHIA studies (left side of Figure \ref{5.multiplicitycomparison}), and confirmed in the multiplicity comparison between minimum bias simulation and triggered data (right side in Figure \ref{5.multiplicitycomparison}). Despite this fact, the $\pi^{0}$ reconstruction shows good agreement between simulation and data, as illustrated in Figure \ref{5.comparisonsimu}. On the other hand, another known and expected difference comes from the invariant mass distribution, and in particular in the background component. As shown in Figure \ref{5.masse}, in fact, while the $\pi^{0}$ peak appears to be consistent in width with data, the hadronic background is substantially underestimated in simulation. This means that we cannot estimate the signal/background ratio directly from simulation. We will need instead to scale the background component to fit the data or, alternatively, use the information of the shape to estimate how the background behaves below the $\pi^{0}$ peak.

\subsection{Background subtraction}

The first step towards a corrected coincidence probability  is represented by the study of the background below the $\pi^{0}$ peak and its effect on azimuthal correlations. From simulations studies, it is clear that the main background component comes from pairs of a photon with a high energy charged hadron. Such pairs are likely to be originated within the same jet; therefore, they provide a good characterization of the jet itself and they are expected to be as correlated in $\Delta\varphi$ as neutral pions. In order to check this, correlations have been computed between a forward $\pi^{0}$ and a mid-rapidity photon pair selected in the invariant mass window $(0.20<M_{\gamma\gamma}<0.33)\mathrm{\,GeV/c^{2}}$, relatively far from the nominal value of the $\pi^{0}$ mass. Figure \ref{5.emcoff} shows the criteria to select the photon pairs and the inclusive correlations between a forward pion and such mid-rapidity pair. Pairs selected off the pion peak appear to be as much correlated as the pion candidates. Also the signal widths, as extrapolated from the Gaussian fit and indicated in figure, appear to be consistent between the two selections. We can therefore conclude that the hadronic background underlying the $\pi^{0}$ peak in the invariant mass spectrum contains similar informations than the $\pi^{0}$ which does not affect our conclusions.

\begin{figure}\label{5.emcoff}
\begin{tabular}{c c}
\includegraphics[width=0.32\textwidth, clip]{figures/chapter5/off1.eps} &
\includegraphics[width=0.64\textwidth]{figures/chapter5/off2.eps} 
\end{tabular}
\caption{Off-peak analysis. Comparison of azimuthal correlations between a forward $\pi^{0}$ and a mid-rapidity photon pair, where the pair is selected within the $\pi^{0}$ mass window (center) and slightly off-peak (right), as indicated by the invariant mass spectra (left). On the top (bottom) row: p+p (d+Au) interactions. Particles are selected using the higher $p_{T}$ cut.}
\end{figure}


The off-peak correlation is also useful for extracting the background component from the ``peak'' region. The coincidence probability can be in fact disentangled into two components: the $\pi^{0}$-$\pi^{0}$ (signal-signal) component and the $\pi^{0}$-pair (signal-background) component. In order to obtain the first one in the (BEMC) $\pi^{0}$ mass window (peak area) we can subtract from the measured  ``on-peak'' correlation the $\pi^{0}$-background correlation estimated from the off-peak region, where the background is by far the largest component. This can be done using the following formula:

\begin{equation}\label{5.eq.back}
\left.\frac{dN^{\pi^{0}\pi^{0}}}{d(\Delta\varphi)}\right|_{P}=\left[\left.\frac{dN}{d(\Delta\varphi)}\right|_{P}-\left.\frac{dN}{d(\Delta\varphi)}\right|_{O}\cdot\frac{\left.N^{b}\right|_{P}}{\left.N^{b}\right|_{O}}\right]\cdot\left[1-\frac{\left.N^{s}\right|_{O}}{\left.N^{s}\right|_{P}}\cdot\frac{\left.N^{b}\right|_{P}}{\left.N^{b}\right|_{O}}\right]^{-1}
\end{equation}

\begin{figure}\label{5.fitsdata}
\begin{tabular}{c c}
\includegraphics[width=0.32\textwidth, height=0.30\textwidth, clip=]{figures/chapter5/differentFitsSimu.eps} &
\includegraphics[width=0.64\textwidth, height=0.30\textwidth]{figures/chapter5/differentFitsData.eps} 
\end{tabular}
\caption{Left: different components of the p+p invariant mass distribution in simulation are disentangled and fitted separately. Right: different fits for the background component are used to fit $M_{\gamma\gamma}$ in data, together with an ``asymmetric Gaussian'' function used for the peak.}
\end{figure}


In this equation, the azimuthal correlations between two neutral pions (signal-signal correlation: $dN^{\pi^{0}\pi^{0}}/d(\Delta\varphi)|_{P}$), where the mid-rapidity pion is selected in the $\pi^{0}$ mass region (P), is obtained by subtracting from the measured ``on-peak'' correlation ($dN/d(\Delta\varphi)|_{P}$) the $\pi^{0}$-background correlation measured ``off-peak'' ($dN/d(\Delta\varphi)|_{O}$), scaled with the ratio of number of background pairs in the peak region ($N^{b}|_{P}$) and off-peak ($N^{b}|_{O}$) in order to reproduce the amount of background present in the $\pi^{0}$ mass window. The scaling factor on the right-hand side accounts for the possibility that the tail of the $\pi^{0}$ peak extends into the off-mass region. When the $\pi^{0}$ peak is fully contained into the on-peak region ($N^{s}|_{P}=\mathrm{max}$) and no signal pairs are to be found in the off-peak region ($N^{s}|_{O}=0$), the off-peak correlation is a purely $\pi^{0}$-background correlation and the scaling factor reduces to one. This formula has the advantage that it is not necessary to know the signal/background ratio to perform the subtraction. In fact, the only knowledge required is the shape of the signal and background components or, more precisely, the relative percentage of the two distribution (independently) in the two mass regions. These relative proportions ($N^{s}|_{P}/N^{s}|_{O}$ for the signal and $N^{b}|_{P}/N^{b}|_{O}$ for the background) can be estimated in different ways, as illustrated in Figure \ref{5.fitsdata}. One can either integrate or fit the different component of the $M_{\gamma\gamma}$ spectrum in simulation, where they are disentangled. Alternatively, one can fit the $M_{\gamma\gamma}$ distribution obtained from data, using the fitting functions from simulation as guideline. On the right-hand panel of Figure \ref{5.fitsdata} four different fitting functions are tested on data (in black) and compared with the background as obtained from simulation (in green). Since the background component is underestimated in simulation, it has been scaled up to fit the data in the off-peak region\footnote{The hadronic and combinatorial component of the background have been scaled by a factor $1.7$, chosen by performing the Kolmogorov test between simulation and data.}. The peak has been fitted using an ``asymmetric Gaussian'' function (i.e. two half Gaussians sharing the mean value but with different variances), while the background has been fitted with polynomial of $\mathrm{1^{th}}$, $\mathrm{2^{nd}}$ and $\mathrm{4^{th}}$ order and with a $\mathrm{2^{nd}}$ order logarithmic function, the last of which provides the best $\chi^{2}$ when compared to the (scaled) background from simulation. The background estimated from integrating simulated spectra, as well as from this last fit on data, will be used to do the subtraction, while the other fits will be used to estimate the systematic uncertainty of the final (corrected) yield. 

\subsection{Efficiency correction}
Once the prescription to subtract the background has been determined, it is possible to apply an efficiency correction to the azimuthal correlation. The reconstruction efficiency and detector acceptance is calculated by performing an association analysis on the reconstructed pair of clusters. Each cluster is associated with a simulated track pointing to it. When more than one track is pointing to the same cluster, the one contributing with the highest energy fraction to the total cluster energy is selected. The detector acceptance $\epsilon_{acc}$ is calculated as the ratio between reconstructed and simulated neutral pions with pseudo-rapidity $|\eta|<0.9$. The number of reconstructed pions is incremented when a pair of clusters, both within the detector acceptance, are associated with the two decaying photons from the same $\pi^{0}$. The reconstruction efficiency $\epsilon_{rec}$ takes into account, in addition, the quality cut applied to the pion candidate to reduce the background, namely the asymmetry cut $Z_{\gamma\gamma}<0.7$ and the ``quality cut'' which requires the peak tower to carry at least $90\%$ of the cluster energy.
Figure \ref{5.efficiency} shows the $p_{T}$ dependence of the acceptance $\epsilon_{acc}$ and the total efficiency $\epsilon=\epsilon_{acc}\times\epsilon_{rec}$ in p+p and d+Au interactions. The acceptance (and thus the efficiency) is lower at low $p_{T}$, due to a higher background contamination, and at large $p_{T}$ because of the actual opening angle cut applied by the clusterfinder. The efficiency proves to be independent on the multiplicity of the event, which is the main difference between trigger data and minimum bias simulation. However, the distribution of the ``quality variable'' $x=E_{seed}/E_{cluster}$, on which the quality cut is applied, appears to be different from simulation and data. In order to make the two distribution comparable, a Gaussian energy smearing has been applied independently to all BEMC towers before the clustering procedure. Figure \ref{5.quality} shows the effect of different smearing values on the quality variable. This provides access to systematic uncertainties on the value of the efficiency, calculated as the average of the values of the efficiency in the two most plausible cases (second and third panel in Figure \ref{5.quality}), while the other cases provide the limits for the systematic uncertainty. The efficiency, when integrated over the whole $p_{T}$ range, turns out to be $\epsilon_{pp}=0.0974\pm0.0032\mathrm{(stat)}\pm0.0067\mathrm{(syst)}$ (and $\epsilon_{dAu}=0.0854\pm0.0031\mathrm{(stat)}\pm0.0039\mathrm{(syst)}$) for pions with $p_{T}>1.5\mathrm{GeV/c}$, $\epsilon_{pp}=0.0570\pm0.0001\mathrm{(stat)}\pm0.0013\mathrm{(syst)}$ (and $\epsilon_{dAu}=0.0475\pm0.0011\mathrm{(stat)}\pm0.0007\mathrm{(syst)}$) for pions with $p_{T}>1.0\mathrm{\,GeV/c}$.

\begin{figure}\label{5.efficiency}
\begin{tabular}{c c}
\includegraphics[width=0.45\textwidth, height=0.30\textwidth]{figures/chapter5/efficiencyPP.eps} 
\includegraphics[width=0.45\textwidth, height=0.30\textwidth]{figures/chapter5/efficiencyDAU.eps} 
\end{tabular}
\caption{BEMC acceptance and reconstruction efficiency for $\pi^0$ candidates in p+p (left) and d+Au interaction (right) as function of $p_{T}$.}
\end{figure}

\begin{figure}\label{5.quality}
\begin{tabular}{c}
\includegraphics[width=0.90\textwidth]{figures/chapter5/quality.eps} 
\end{tabular}
\caption{Simulation-Data comparison between the ``quality cut'' ratio $E_{seed}/E_{cluster}$ for different values of the tower energy smearing for p+p interactions (higher $p_{T}$ selection).}
\end{figure}


\subsection{Systematics}
Once the BEMC reconstruction efficiency is estimated, it is possible to correct the coincidence probability between a forward $\pi^{0}$ and a mid-rapidity $\pi^{0}$. The two-step process consists first in subtracting the $\pi^{0}$-background contribution from the azimuthal correlation, using Equation \ref{5.eq.back}, and then scale it for the $\pi^{0}$ efficiency. As for the FMS-TPC correlations, the correlation obtained is fitted with a constant background plus a periodic Gaussian centered in $\Delta\varphi=\pi$, so that the correlated yield can be extracted as the area of the Gaussian function. We estimated the shape of signal and background in the $\pi^{0}$ invariant mass by fitting the histogram components from simulation (left-hand side of Figure \ref{5.fitsdata}) and we scale the correlation so obtained by an overall efficiency factor, integrated over $p_{T}$, indicated in the previous section. The correlated yield for p+p (and d+Au) calculated in this way reads:      
$A_{pp}=0.023\pm0.002$ ($A_{dAu}=0.025\pm0.004$) for higher $p_{T}$ cuts ($p_{T}^{FMS}>2.5\mathrm{\,GeV/c}$, $p_{T}^{FMS}>p_{T}^{EMC}>1.5\mathrm{\,GeV/c}$)  and $A_{pp}=0.059\pm0.003$ ($A_{dAu}=0.067\pm0.014$) for lower $p_{T}$ cuts ($p_{T}^{FMS}>2.0\mathrm{\,GeV/c}$, $p_{T}^{FMS}>p_{T}^{EMC}>1.0\mathrm{\,GeV/c}$). However, due to the larger uncertainties affecting the FMS-BEMC measurement, a number of additional checks have been performed in order to extract the correlated yield. These include different efficiency and background estimates, checks on data sanity and kinematical cuts. They are listed below, while the values for the correlated yield in all cases are summarized at the end (Table \ref{5.syssum}. This first reference measurement is labeled as Check n.0).

\begin{description}
\item[1. Transverse momentum weighted efficiency.]
The $p_{T}$ distribution of mid-rapidity pions is well described by simulation (Figure \ref{5. comparisonsimu}). Therefore we are entitled to use an overall efficiency factor, integrated over the whole $p_{T}$ range. However, a different approach can be to estimate the efficiency for single $p_{T}$ bins and to weight them using the $p_{T}$ distribution from data. This leads again to a single efficiency factor, which does not differ much from the value used in the reference measurement. 

\item[2. Transverse momentum dependent efficiency and background.]
A similar approach consists in performing the efficiency correction (and, before that, the background subtraction) for each single $p_{T}$ bin. In this way the background component is estimated (as before, from fit on simulation) in each bin and the efficiency correction is applied accordingly.The total azimuthal correlation is eventually obtained by summing all these components. 

\item[3. Cluster ``quality cut''.]
In order to test the consistency of the variable $E_{seed}/E_{cluster}$, efficiency and (fitted) background have been estimated using the stricter condition $E_{seed}/E_{cluster}>95\%$. 
Analogously we calculated the correlated yield for $\pi^{0}$ correlations where no ``quality cut'' has been used to select the clusters.
  
\item[4. Energy asymmetry.]
A check on the energy asymmetry cut has been performed by requiring a stricter ($Z_{\gamma\gamma}<0.5$) condition. 

\item[5. Background correction with different $M_{\gamma\gamma}$ windows.]
The larger uncertainty in measurement of the $\pi^{0}$-$\pi^{0}$ correlation is represented by the quantification of the background component in the BEMC $M_{\gamma\gamma}$ spectrum. For this reason, a series of different methods to estimate the background below the $\pi^{0}$ peak have been pursued. At first, we can use a different invariant mass window to define the off-mass pair in the usual formula \ref{5.eq.back}. Instead of estimating the correlated background from correlations with a pair in the region $(0.20<M_{\gamma\gamma}<0.33)\mathrm{\,GeV/c^{2}}$, we use the further region $(0.33<M_{\gamma\gamma}<0.46)\mathrm{\,GeV/c^{2}}$. In this case, the efficiency and the background shape from simulation stay the same as in the reference measurement.  

\item[6. Background correction with $M_{\gamma\gamma}$ windows based on resolution.]
A different background estimate can be achieved by select $M_{\gamma\gamma}$ windows based on the peak mean value and its resolution. Data show that the $\pi^{0}$ peak in the invariant mass spectrum in data ($\mu=(0.139+0.031-0.026)\mathrm{\,GeV/c^{2}}$ for hight $p_{T}$ p+p interaction)\footnote{The asymmetry in the signal width is due to the ``asymmetric Gaussian'' used for the fit.} is both broader than in simulation ($\mu=(0.131+0.032-0.020)\mathrm{\,GeV/c^{2}}$ for the same set); moreover, its position is centered in a slightly different mean value. In order to make the selection consistent between data and simulation, cluster pairs in the invariant mass spectra have been selected in the two regions $\left[\mu-2.7\sigma_{-};\mu+1.9\sigma_{+}\right]$ for the peak and $\left[\mu+1.9\sigma_{+};\mu+6.1\sigma_{+}\right]$ for the off-mass selection. 
 
\item[7. Background estimated from integrals in simulation.]
Instead of estimating signal and background in the invariant mass spectrum by fitting the different component in simulation, one can take directly the integrals of such components in the $M_{\gamma\gamma}$ regions of interest. As shown in Figure \ref{5. fitsdata} (left panel), the difference between fit and histograms is particularly significant for low mass values in the hadronic background and the tail of the signal peak in the off-mass region ($M_{\gamma\gamma}>0.20\mathrm{\,GeV/c^{2}}$).  

\item[8. Background estimated from fit on data.]
Alternatively, one can estimate the signal and the background shapes by fitting the invariant mass spectrum obtained from data. As shown in the right-hand panel of Figure \ref{5.fitsdata}, the fitting function (on data) that best represents the (scaled) background shape from simulation is a second-order logarithmic function. Another fitting function that provide a reasonable comparison with simulated background is the fourth-order polynomial. As an limit case, we can fit the invariant mass on data using either a first-order or a second-order polynomial. In the first case the background is overestimated in comparison with simulation. In the second case (but only for higher $p_{T}$ selections) the background is underestimated.
 

\end{description}     
 

\begin{table}\label{5.syssum}
\begin{tabular}{c c}
\begin{tabular}{| c | c  | c |}
\hline Check & $A_{pp}$ & $A_{dAu}$\\ \hline \hline
0 & 0.023$\pm$0.002 & 0.025$\pm$0.004 \\ \hline
1 & 0.024$\pm$0.002 & 0.026$\pm$0.004 \\ \hline
2 & 0.023$\pm$0.007 & 0.026$\pm$0.007 \\ \hline
\multirow{2}{*}{3} &  0.027$\pm$0.002 & 0.023$\pm$0.004 \\ \cline{2-3}
&  0.023$\pm$0.001 & 0.025$\pm$0.004 \\ \hline
4 & 0.027$\pm$0.002 & 0.022$\pm$0.005 \\ \hline
5 & 0.023$\pm$0.002 & 0.025$\pm$0.003 \\ \hline
6 & 0.025$\pm$0.002 & 0.028$\pm$0.004 \\ \hline
7 & 0.022$\pm$0.002 & 0.023$\pm$0.004 \\ \hline
\multirow{4}{*}{8} &  0.022$\pm$0.002 & 0.024$\pm$0.003 \\ \cline{2-3}
&  0.022$\pm$0.002 & 0.025$\pm$0.004 \\ \cline{2-3}
&  0.018$\pm$0.002 & 0.020$\pm$0.003 \\ \cline{2-3}
&  0.027$\pm$0.002 & 0.033$\pm$0.004 \\ \hline
\end{tabular}
&
\begin{tabular}{| c | c  | c |}
\hline Check & $A_{pp}$ & $A_{dAu}$\\ \hline \hline
0 & 0.059$\pm$0.003 & 0.067$\pm$0.014 \\ \hline
1 & 0.064$\pm$0.004 & 0.067$\pm$0.014 \\ \hline
2 & 0.066$\pm$0.019 & 0.067$\pm$0.031 \\ \hline
\multirow{2}{*}{3} &  0.066$\pm$0.005 & 0.070$\pm$0.014 \\ \cline{2-3}
&  0.060$\pm$0.003 & 0.060$\pm$0.003 \\ \hline
4 & 0.060$\pm$0.004 & 0.061$\pm$0.005 \\ \hline
5 & 0.056$\pm$0.003 & 0.070$\pm$0.010 \\ \hline
6 & 0.067$\pm$0.003 & 0.067$\pm$0.014 \\ \hline
7 & 0.060$\pm$0.003 & 0.067$\pm$0.014 \\ \hline
\multirow{4}{*}{8} &  0.056$\pm$0.003 & 0.063$\pm$0.004 \\ \cline{2-3}
&  0.053$\pm$0.005 & 0.067$\pm$0.014 \\ \cline{2-3}
&  0.055$\pm$0.003 & 0.067$\pm$0.010 \\ \cline{2-3}
&  0.048$\pm$0.004 & 0.063$\pm$0.011 \\ \hline
\end{tabular}
\end{tabular}
\caption{Summary of the systematic analysis for the extraction of the correlated yield in p+p and d+Au interactions for higher (left panel) and lower (right panel) $p_{T}$ selections.}
\end{table}


This procedure provide access to the systematic uncertainty on the value of the correlated yield. The main contribution to such uncertainty is carried by the background estimation. The expected value for the correlated yield and its statistical errors are taken from a fit on all the contributions. The systematic uncertainty range is conservatively defined by the two outermost values found in the study. This lead to the following values for the correlated yield: $A_{pp}=0.024\pm0.001^{+0.003}_{-0.006}$ ($A_{dAu}=0.025\pm0.001^{+0.008}_{-0.005}$) for higher $p_{T}$ cuts, $A_{pp}=0.058\pm0.001^{+0.009}_{-0.010}$ ($A_{dAu}=0.062\pm0.002^{+0.008}_{-0.003}$) for lower $p_{T}$ cuts. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





